Meta-Learning by the Baldwin Effect

The scope of the Baldwin effect was recently called into question by two papers that closely examined the seminal work of Hinton and Nowlan. To this date there has been no demonstration of its necessity in empirically challenging tasks. Here we show that the Baldwin effect is capable of evolving few-shot supervised and reinforcement learning mechanisms, by shaping the hyperparameters and the initial parameters of deep learning algorithms. Furthermore it can genetically accommodate strong learning biases on the same set of problems as a recent machine learning algorithm called MAML "Model Agnostic Meta-Learning" which uses second-order gradients instead of evolution to learn a set of reference parameters (initial weights) that can allow rapid adaptation to tasks sampled from a distribution. Whilst in simple cases MAML is more data efficient than the Baldwin effect, the Baldwin effect is more general in that it does not require gradients to be backpropagated to the reference parameters or hyperparameters, and permits effectively any number of gradient updates in the inner loop. The Baldwin effect learns strong learning dependent biases, rather than purely genetically accommodating fixed behaviours in a learning independent manner.

==> ga_pseudo.tex <==
\begin{algorithm}[t]
\caption{Generational Genetic Algorithm}
\label{alg:gga}
\begin{algorithmic}[1]
\REQUIRE $\mathcal{S}$: size of the population
\REQUIRE $\population$: initial population-representation of individuals (of size $\mathcal{S}$)
%\REQUIRE $\mathcal{P}_{next}$: representation of the next generation of population
\REQUIRE $\mathcal{E}$: Percentage of best individuals carried over to next generation (elitism)
\REQUIRE $\fitness$: fitness scoring function
\WHILE{not done}
\FORALL{$g \in \population$}
\STATE Evaluate genotype: $V[g] \leftarrow \fitness(g)$
\ENDFOR
\STATE Sort genotypes according to increasing fitness: $\population, V \leftarrow sort(P, V, key=V)$
\FOR{$\texttt{k=1...}\mathcal{S}$}
\STATE Assign ranks to the genotypes: $R[V[k]] \leftarrow k$.
\ENDFOR
\STATE Copy best genotypes:
\FOR{$\texttt{k=1...}\mathcal{S} * \mathcal{E}$}
  \STATE $\population_{next}[k] \leftarrow \population[S - k + 1]$
\ENDFOR

\STATE Select the remainining surviving genotypes based on rank:
\FOR{$\textt{k=}\mathcal{S} * \mathcal{E} + 1...\mathcal{S}$}
  \STATE $\population_{next}[k] \leftarrow \textt{choice}(\population, \textt{weight=}R)$
\ENDFOR

 \STATE Update population based on fitness of individuals:\newline
 $\population \leftarrow \popupdate(\population,\{\left(1,{\theta^1},\alpha^1,f^1\right),..., \left(g,{\theta^g}, \alpha^g,f^g\right)\}$)
\ENDWHILE
%\STATE while 
\end{algorithmic}
\end{algorithm}
